Hilbert functions of points on Schubert varieties in Orthogonal Grassmannians

A solution is given to the following problem: how to compute the multiplicity, or more generally the Hilbert function, at a point on a Schubert variety in an orthogonal Grassmannian. Standard monomial theory is applied to translate the problem from geometry to combinatorics. The solution of the resulting combinatorial problem forms the bulk of the paper. This approach has been followed earlier to solve the same problem for the Grassmannian and the symplectic Grassmannian. As an application, we present an interpretation of the multiplicity as the number of non-intersecting lattice paths of a certain kind. Taking the Schubert variety to be of a special kind and the point to be the "identity coset," our problem specializes to a problem about Pfaffian ideals treatments of which by different methods exist in the literature. Also available in the literature is a geometric solution when the point is a "generic singularity."

==> amsart-title.tex <==
\title[Schubert varieties in Orthogonal Grassmannians]%
{Hilbert functions of points on\\
	Schubert varieties in Orthogonal Grassmannians}
\author{K.~N.~Raghavan}
	\address{Institute of Mathematical Sciences, C.~I.~T.~Campus\newline
		\hbox{\hspace{\parindent}}%
		Chennai 600\,113, INDIA}
	\email{knr@imsc.res.in}
\author{Shyamashree Upadhyay}
	\address{Chennai Mathematical Institute,
		Plot No. H1, SIPCOT IT Park\newline
		\hbox{\hspace{\parindent}}%
		Padur Post, Siruseri 603\,103,	Tamilnadu, INDIA}
	\email{shyama@cmi.ac.in}
\subjclass[2000]{Primary: 05E15, Secondary: 13F50, 13P10, 14L35}


==> erratum.tex <==
\mysubsectionstar{Erratum}\mylabel{s.erratum}
\addcontentsline{toc}{subsection}{Erratum}
\begin{itemize}
\item
In the very last proof of the paper,  the very last line of page~69 has
been changed.   The element~$\alpha$ could be any element of intersection,
not just the topmost.   This has been taken care of in the cvs version
titled {\ttfamily correction-1}.    

\item
Page~41, line~4: $\opi$ should be replaced by $\ophi$. (corrected)
\end{itemize}

==> groebner.tex <==
\mysection{Computation of the initial ideal}%
\mylabel{s.groebner}\mylabel{s.initial}
Fix $v\leq w$ in $I(d)$.
Recall from~\S\ref{sss.smttgtcone} that the affine patch $\miso\cap\affinev^v$
of $\miso$ defined by the non-vanishing of the projective co-ordinate~$q_v$
can be identified with the affine space with co-ordinates~$X_{(r,c)}$ for
$(r,c)\in\oroots$.      Under this identification,  the point $\pointe^v$
corresponds to the origin of the affine space.
The ideal---let us denote it $I$---of
the tangent cone at $\pointe^v$ to the Schubert variety~$X(w)$ is generated by 
$\{f_\tau\st \tau\in I(d),\tau\not\leq w\}$---note that 
$f_\tau(:=q_\tau/q_v)$ is a homogeneous polynomial in the~$X_{(r,c)}$ 
of degree the
cardinality of $v\setminus\theta$.     
Computed below is the initial ideal of $I$ with respect to a suitable
term order on the set of monomials in~$\oroots$ (more precisely on
$X_{(r,c)}$ but it is convenient to abuse notation and not distinguish
$(r,c)$ from $X_{(r,c)}$).

\mysubsection{The term order}\mylabel{ss.termorder}
We denote by $>$ our term order on monomials in~$\oroots$ and 
prescribe it now in several steps.   
The terminology and notation of \cite[\S15.2]{ebud} are in force.
Let $\mon$ and $\mont$ be monomials in $\oroots$.   
\begin{itemize}
\item 
If $\deg\mon>\deg\mont$ then $\mon>\mont$.    
\item
If $\deg\mon\cap\posv>\deg\mont\cap\posv$ then $\mon>\mont$.
\item
Suppose that $\deg\mon\cap\posv=\deg\mont\cap\posv$.   Then look at
the set of projections (both vertical and horizontal) on the diagonal
of elements of $\mon\cap\posv$ and $\mont\cap\posv$---some of these
projections may be only in $\and\roots\modv$ and not in $\and\pos\modv$.
Let $r_1\geq \ldots\geq r_{2k}$ and $r'_1\geq\ldots\geq
r'_{2k}$ be respectively the row numbers of these projections
for $\mon$ and $\mont$.    If the two
sequences are different,  then $\mon>\mont$ if $r_j>r'_j$ for the least
$j$ such that $r_j\neq r'_j$. 
\item Suppose that the projections on the diagonal of 
$\mon\cap\posv$ and $\mont\cap\posv$ are the same.   Consider the
column numbers of elements in both $\mon\cap\posv$ and $\mont\cap\posv$ 
that give rise to the projection with the least row number (namely
$r_{2k}=r'_{2k}$).    Suppose
$c_1\geq\ldots\geq c_\ell$ and $c'_1\geq\ldots\geq c'_\ell$ are these
numbers respectively for $\mon\cap\posv$ and $\mont\cap\posv$.   If
these sequences are different,  then $\mon>\mont$ if $c_j\geq c'_j$
for the least $j$ such that $c_j\neq c'_j$.    If the sequences are
the same then there is an equality of 
sub-monomials of $\mon$ and $\mont$ consisting of
those elements with row numbers $r_{2k}=r'_{2k}$.   We remove this
sub-monomial from both $\mon$ and $\mont$ and then appeal to an induction
on the degree.
\item
Finally, to deal with the case $\mon\cap\posv=\mont\cap\posv$, 
we fix an arbitrary
total order on $\oroots\setminus\posv$ and prescribe the restriction of
$>$ to monomials in $\oroots\setminus\posv$ to be the degree-lexicographic
order induced from this total order.
\end{itemize}
%This finishes the description of the term order~$>$.

\mysubsection{Statement of the result}\mylabel{ss.result}
Let $P$ denote the polynomial ring $\field[X_\beta\st\beta\in\oroots]$,
the co-ordinate ring of the affine patch $\miso\cap\affinev^v$ (here $\field$
denotes the underlying field).
For $J$ an ideal in~$P$, 
denote by $\init J$ the ideal generated by the initial terms,
with respect to the term order~$>$ defined above,
of elements of $J$.    
The Hilbert functions of the graded rings
$P/I$ and $P/\init I$ being the same,  it follows
from Theorem~\ref{t.main} that the graded piece of degree~$m$ of $P/\init I$
has dimension the cardinality of the set $\svwm$ of $w$-dominated
monomials in $\oroots$ of degree~$m$.      
\begin{proposition}\mylabel{p.groebner}
  Every monomial in $\oroots$ that is not $w$-dominated belongs to
$\init I'$ where $I'$ is the ideal of $P$ generated by 
$\{f_\tau\st \tau\in\id, v\leq\tau\not\leq w\}$.
\end{proposition}
As an immediate consequence of the proposition,  we have
\begin{corollary}\mylabel{c.p.groebner}
  The natural map $P/\init I'\twoheadrightarrow P/\init I$ is an isomorphism.
In particular,  the ideals $I'$ and $I$ are equal.
\end{corollary}
\mysubsection{Proof of Proposition~\ref{p.groebner}}\mylabel{ss.pf.p.groebner}
\endinput
Here we interpret Theorem~\ref{tmain} 
in terms of Gr\"obner basis---see Proposition~\ref{p.grob}
below.     The special case of the proposition when $v$ is
the identity coset (that is, $v=(1,\ldots,d)$)
has been obtained by~?? by different methods.
\marginpar{Put in correct reference(s).}

Fix elements $v,w$ in $I(d)$ with $v\leq w$. 
Recall from \S\ref{ssmt} that the ideal
$$
\left(f_\theta=q_\theta/q_v\st \theta\nleq w\}\right)
$$ 
in the polynomial ring $P:=k[X_\beta\st\beta\in\oroots^v]$ defines the 
tangent cone to the Schubert variety $X_w$ at the point $e^v$.   
We will identify a subset of these generators~$q_\theta$ as being Gr\"obner
basis with respect to certain term orders for the ideal of the tangent cone.
Observe that the $q_\theta$ are homogeneous polynomials in the
variables $X_\beta$.

\begin{figure}
\begin{center}
\mbox{\epsfig{file=fextwo.eps,height=5cm,width=12.5cm}}
\caption{\label{fextwo}All the symmetric tuples of non-intersecting 
lattice paths as in Example~\ref{etwo}}
\end{center}
\end{figure}

Let us call an element $\theta$ of $I(d)$ {\em good\/} (the scope of
this terminology is intended to be limited to this section) if the
\begin{itemize}
\item $v\leq u$ and $t\nleq w$;
% \item $\mon_\theta=\mon_\theta^\text{up}$,  that is,
% $r\leq c^*$ for $(r,c)$ in $\mon_\theta$,  and the elements of 
% $\mon_\theta$ form a $v$-chain---here $\mon_\theta$ is the monomial
% attached to $\theta$ as in Proposition~\ref{poldmonw}.\footnote{
% While it is true that in
% \S\ref{sproofcompletion} we are using the notation of \cite{kr}
% where the symbols have a different meaning from what they do in \S\ref{stheorem}--\ref{sfurtherred},
% the condition that $r\leq c^*$ for $(r,c)$ in $\mon_\theta$ gives
% us some license for sloppiness.}
monomial $\Phi_w^\star$ is a \vchain\ in $\posv$,  where, in keeping
with the notation of \S\ref{s.ophi},  $Phi_w^\star$ denotes the result
of applying $\ophi$ to the pair $(\theta,\Phi)$ where $\Phi$
denotes the empty monomial.
Let $\ap=(t,u)$ be an admissible pair and $(\theta,\theta^\hash)$
the pair associated to $\ap$ as in Proposition~\ref{pap}.  
Let us call $\ap$ ``good'' (the scope of this
terminology is intended to be limited to this section) if 
\end{itemize}

Suppose that $\ap$ is good.   Then $\mon_\theta$ occurs up to sign
as a term in the expression for $f_\ap=f_\theta$ as the determinant
of a submatrix of the matrix of the form on page~\pageref{pagematrix}
attached to $v$---here we are abusing notation and not distinguishing
between a monomial in $\oroots^v$ and the corresponding monomial
in the variables $X_\beta$, $\beta$ in $\oroots^v$.

\bprop\label{pgrob}\label{pgroebner}
Fix elements $v\leq w$ of $I(d)$. Fix any term order on the
monomials in the standard graded
polynomial ring $P:=k[X_\beta\st\beta\in\oroots^v]$ such
that, for any good admissible pair $\ap$,  the initial term of
$f_\ap$ 
is $\mon_\theta$. 
Then the\/
$f_\ap$ as $\ap$ varies over all good admissible pairs
form a Gr\"obner basis
with respect to this term order for the ideal
$(f_\ap\st
\ap\text{ admissible pair, } \aptop{\ap}\nleq w)$
defining the
tangent cone to the Schubert variety $X_w$ at the point $e^v$.\eprop
\bproof   
Denoting by $I$ the ideal
$(f_\ap\st\ap\text{ admissible pair,
$\aptop{\ap}\nleq w$})$ defining the tangent cone, 
by $\init{f}$ the
initial term of a polynomial $f$ in the fixed term order,  and by $\init{I}$
the ideal $\left(\init{f}\st f\in I\right)$,  we clearly have a graded
surjection
\[
P/
\left(
\init{f_\ap}\st\ap\text{ good admissible pair,
$\aptop{\ap}\nleq w$}\right) 
\surjection P/\init{I}
\]
The assertion is that this map is an isomorphism. To 
prove this,  it is enough to show that the Hilbert function
of the quotient ring dominates that of the ring on the left.

The Hilbert function of $P/\init{I}$ is the same as that of the tangent cone
$P/I$,  and so by Theorem~\ref{tmain} its value at a positive
integer $m$ is the cardinality of
the set $\svwm$ of $w$-dominated
monomials in $\oroots^v$ of degree $m$.  It therefore suffices to
observe that a monomial
in $\oroots^v$ that is not $w$-dominated belongs to the ideal
$\left(
\init{f_\ap}\st\ap\text{ good admissible pair,
$\aptop{\ap}\nleq w$}\right)$.
Given such a monomial, choose a $v$-chain
$\beta_1>\ldots>\beta_t$ in it
such that $w\ngeq s_{\beta_1}\cdots s_{\beta_t}v$.  Applying the lemma below
to the this $v$-chain,  we get a good admissible pair $\ap$ such that
the initial term of $f_\ap$ in the fixed term order is
$\{\beta_1,\ldots,\beta_t\}$.\eproof
\blemma\label{lgrob}
Fix elements $v\leq w$ of $I(d)$.
Let 
$\beta_1>\ldots>\beta_r$ be a $v$-chain of elements in $\pos^v$
such that $w\ngeq s_{\beta_1}\cdots s_{\beta_r}v$.
The element of\/
${\rm SM}^{v,v}$\/ that corresponds under the bijection of
Proposition~\ref{pbijection} to the element 
$\{\beta_1,\ldots,\beta_r\}$ of\/ $T^v$
consists of a single admissible pair $\ap=(t,u)$ which is good and for which
$\mon_\theta=\{\beta_1,\ldots,\beta_r\}$.
\elemma

\bproof
We follow the notation of the statement and
proof of Proposition~\ref{pbijection}.    
Set $\mon =\{\beta_1,\ldots,\beta_r\}
\cup\{\beta_1^\hash,\ldots,\beta_r^\hash\}$,   $\pi(\mon)=(t,\mon')$,
and $\pi(\mon')=(u,\min)$.      We know from that
proposition that $(t,u)$ is an admissible pair and that
$v\leq u$.    Since the bijection ${\rm SM}^{v,v}\simeq T^v$ respects
domination,   and $s_{\beta_1}\cdots s_{\beta_r}v\nleq w$ by hypothesis,
it follows that $t\nleq w$.    It remains to be seen that
$\min$ is the empty monomial and
that $\mon_\theta=\{\beta_1,\ldots,\beta_r\}$.  These will follow from 
explicit computation which we now perform.

Set $\beta_j=(r_j,c_j)$;  then
$\beta_j^\hash=(c_j^*,r_j^*)$. 
Since $\beta_j\in\pos^v$,  we have $c_j\leq r_j^*$ and $c_j<r_j$,  and so
$\{c_1,\ldots,c_t\}\subseteq [d]$. 

Consider the two-step partitioning of $\mon$ into the $\mon_j$
and the $\mon_j$ into blocks.   It is readily seen that
$\mon_j=\{\beta_j,\beta_j^\hash\}$.
Let $s$ be the largest integer, $0\leq s\leq r$, 
such that $r_s\geq r_s^*$---set
$s=0$ if $r_1<r_1^*$.    In other words,
$s$ is the least integer, $0\leq s\leq t$, such that 
$\{r_{s+1},\ldots,r_t\}\subseteq [d]$. 
For $1\leq j\leq s$,   $\mon_j$ is a single block.   For $s<j\leq t$,
the block decomposition of $\mon_j$ is
$\{\beta_j\}\cup\{\beta_j^\hash\}$.

The following expressions for $\mon'$, $u$, $t$, and $\min$
follow readily from 
the definition of the map $\pi$:
$$
\mon'  =  \{(r_1,r_1^*),\ldots,(r_t,r_t^*)\} \quad {\rm and} \quad 
u  =  \left( v\cup\{r_{1},\ldots,r_s\}\right)
	\setminus \left( \{r_{1}^*,\ldots,r_s^*\}\right),
$$
and 
\[ %\begin{array}{c}
t  =  \left( v\cup\{c_1^*,\ldots,c_t^*\}\cup\{r_{s+1},\ldots,r_t\} \right)
  \setminus \left( \{c_1,\ldots,c_t\}\cup\{r_{s+1}^*,\ldots,r_t^*\} \right),
									\]
and $\min$ is the empty monomial.   Now, upon letting $[d]^{\rm c}:=\{d+1,\ldots,2d\}$, put
$$
\theta :=  \left(t\cap [d] \right)\cup \left( u\cap [d]^{\rm c} \right) = 
\left( v\cup\{r_1,\ldots,r_t\}\right)	\setminus\{c_1,\ldots,c_t\}
$$
and
$$
\theta^\hash :=  \left(u \cap [d] \right)\cup \left( t \cap \right [d]^{\rm c}) = 
\left(v\cup\{c_1^*,\ldots,c_t^*\}\right) \setminus\{r_1^*,\ldots,r_t^*\}.
$$
Immediately from the definition of $\mon_\theta$,  we have
\[ 
\mon_\theta=\{(r_1,c_1),\ldots,(r_t,c_t)\}\quad\text{and}\quad
 \mon_{\theta^\hash}=\{(c_1^*,r_1^*),\ldots,(c_t^*,r_t^*)\}. %\Box 
\]
Thus the lemma is proved.
%\eprooftwo
\eproof


We finish by listing some term orders that satisfy the requirement
of Proposition~\ref{pgroebner}.    Fix notation and
terminology as in \S15.2 of \cite{ebud}.  Defined below are
eight total orders $\poone$ through $\po_8$ 
on the elements of $\pos^v$.  Let $>_j$ denote also any
total order on $\oroots^v$ that refines the total order $>_j$ on $\pos^v$.
The homogeneous
lexicographic orders induced by $\poone$,  $\potwo$, $\po_7$, $\po_8$
and the
reverse lexicographic orders induced by $\po_4$, $\po_6$ 
satisfy the requirement of Proposition~\ref{pgroebner}.   The reverse
lexicographic orders induced by $\po_3$, $\po_5$ do not satisfy the requirement.

The total orders $\poone$ through $\po_8$ on $\pos^v$ are as follows:
	for $(r,c)$ in $\pos^v$ and $(a,b)$ in $\oroots^v\setminus\pos^v$,
	\begin{enumerate}
	\item	$(r,c)\poone(r',c')$ if either (a)~$r<r'$ or
			(b)~$r=r'$ and $c>c'$.
	\item	$(r,c)\potwo(r',c')$ if either (a)~$c>c'$ or
			(b)~$c=c'$ and $r<r'$.
	\item	$(r,c)\pothree(r',c')$ if either (a)~$r<r'$ or
			(b)~$r=r'$ and $c<c'$.
	\item	$(r,c)\pofour(r',c')$ if either (a)~$c>c'$ or
			(b)~$c=c'$ and $r>r'$.
	\item	$(r,c)\po_5(r',c')$ if either (a)~$c<c'$ or
			(b)~$c=c'$ and $r<r'$.
	\item	$(r,c)\po_6(r',c')$ if either (a)~$r>r'$ or
			(b)~$r=r'$ and $c>c'$.
	\item	$(r,c)\po_7(r',c')$ if either (a)~$c<c'$ or
			(b)~$c=c'$ and $r>r'$.
	\item	$(r,c)\po_8(r',c')$ if either (a)~$r>r'$ or
			(b)~$r=r'$ and $c<c'$.
			\end{enumerate}


==> old-index.tex <==
\begin{theindex}

  \item $>$, relation on $\posv$\dotfill 10
  \item $\leq$, partial order on $I(d,2d)$\dotfill 9

  \indexspace

  \item $\affinev$, affine patch $q_v\neq 0$ of $\miso$\dotfill 13
  \item $\alpha\down$, for $\alpha\in\andposv$\dotfill 24
  \item $\alpha^\hash$ for $\alpha$ in $\andposv$\dotfill 21
  \item $\alpha\up$, for $\alpha\in\andposv$\dotfill 24
  \item anti-domination\dotfill 17

  \indexspace

  \item $B$, a specific Borel subgroup\dotfill 7
  \item $\bfinish$, for $\beta\in\mon_w\up$\dotfill 64
  \item $\bstart$, for $\beta\in\mon_w\up$\dotfill 64
  \item block
    \subitem in the sense of ~\cite{kr}\dotfill 46
    \subitem of a monomial $\mon$ in $\posv$\dotfill 50

  \indexspace

  \item comparability, of elements of $\roots$\dotfill 28
  \item connected components of a \vchain\dotfill 22
  \item connectedness of two succcessive elements in a $v$-chain\dotfill 
		21
  \item critical element (of a $v$-chain)\dotfill 23

  \indexspace

  \item $d$, integral part of $n/2$ (unfortunately also used otherwise)\dotfill 
		6, 8
  \item degree, of a monomial\dotfill 9
  \item degree, of a standard monomial\dotfill 15
  \item $\delta_j$, for $j$ odd\dotfill 43
  \item depth (of an element $\alpha$ in a monomial $\mon$ in~$\andposv$) = $\depthin{\mon}{\alpha}$\dotfill 
		45
  \item depth (of a monomial $\mon$ in $\andposv$)\dotfill 45
  \item diagonal, $\diagv $\dotfill 9, 10
  \item distinguished (a subset of $\andposv$)\dotfill 20
  \item domination (among elements of $\roots$)\dotfill 28
  \item domination map\dotfill 17

  \indexspace

  \item $e_1,\ldots,e_n$, a specific basis of $V$\dotfill 7
  \item $\pointe^v$, $T$-fixed point\dotfill 9

  \indexspace

  \item $\langle\ ,\ \rangle$, bilinear form on $V$\dotfill 6
  \item $f_\theta:=q_\theta/q_v$\dotfill 13

  \indexspace

  \item head, of a $v$-chain\dotfill 10
  \item horizontal projection $p_h(\alpha)$\dotfill 21

  \indexspace

  \item $\id$\dotfill 9
  \item $I(d,2d)$\dotfill 9
  \item $i\even$, for an integer $i$\dotfill 28
  \item $i\odd$, for an integer $i$\dotfill 28
  \item intersection (of a monomial in a set with a subset)\dotfill 10
  \item isotropic subspace\dotfill 6
  \item $\isubn$\dotfill 7
  \item $\isubn'$\dotfill 7

  \indexspace

  \item $\field$, base field, ($\textup{characteristic}\neq2$)\dotfill 
		6, 14
  \item $k^*(:=n+1-k)$\dotfill 6, 9

  \indexspace

  \item $L$, line bundle\dotfill 12
  \item $\path_\beta$, for $\beta\in\mon_w\up$\dotfill 65
  \item lattice path, from $\bstart$ to $\bfinish$, denoted $\path_\beta$\dotfill 
		64
  \item legs of $\alpha$, for $\alpha\in\posv$\dotfill 21
  \item legs, intertwining of\dotfill 21
  \item length, of a $v$-chain\dotfill 10

  \indexspace

  \item $\miso$, orthogonal Grassmannian\dotfill 6, 7
  \item $\miso'$\dotfill 6
  \item monomial\dotfill 9
  \item $\monomvw$\dotfill 68
  \item multiplicity, of $X(w)$ at $\pointe^v$\dotfill 64
  \item $\textup{multiset}:=\textup{monomial}$\dotfill 9

  \indexspace

  \item $\andposv $\dotfill 9
  \item $n:=\dim V$, (even from \S\ref{ss.basicnotn} on)\dotfill 6, 8

  \indexspace

  \item ${\rm O}(V)$\dotfill 6
  \item $\ortho$-depth\dotfill 26
  \item $\posv $\dotfill 9
  \item $\opbstar$\dotfill 43
  \item $\ophi$\dotfill 16, 41
  \item $\opi$\dotfill 16, 33, 34
  \item $\rootsv $\dotfill 9
  \item $\ortho$-domination\dotfill 10
  \item orthogonal Grassmannian ($\miso$)\dotfill 6

  \indexspace

  \item $\pathsvw$\dotfill 65
  \item $\pbeta$\dotfill 42
  \item $\pbstar$\dotfill 42
  \item Pfaffian $q_\theta$\dotfill 13
  \item $p_h(\alpha)$, horizontal projection\dotfill 21
  \item piece of $\mont$ (see also caution)\dotfill 42
  \item $p_\theta$, Pl\"ucker coordinate\dotfill 12
  \item $p_v(\alpha)$, vertical projection\dotfill 21

  \indexspace

  \item $\myrho_{C,\alpha}$, for $\alpha$ in a \vchain~$C$\dotfill 23
  \item $q_\theta$, Pfaffian\dotfill 13

  \indexspace

  \item $\androotsv$\dotfill 9

  \indexspace

  \item $\mon$, fixed monomial in $\posv$ in~\S\ref{s.opi},~\S\ref{ss.l.ortho}%\dotfill 
		\ignore{50}
  \item $\sv$, set of monomials in $\rootsv$\dotfill 17
    \subitem modifications\dotfill \see{Notation~\ref{n.explain}}{17}
  \item $\mon_C$, where $C$ is a $v$-chain\dotfill 22
  \item $\mon_{C,\alpha}$, for $\alpha$ in a \vchain~$C$\dotfill 23
  \item Schubert varieties\dotfill 6, 7
  \item $\mon\down$, for a monomial $\mon$\dotfill 24
  \item $\mon^\hash$, for monomial $\mon$ in $\andposv$ or $\androotsv$\dotfill 
		21
  \item $\sigma_k$\dotfill 33
  \item $\monjjpone$, for $\mon$ in $\posv$, $j$ odd\dotfill 33
  \item $\monjjponeext$, for $\mon$ in $\posv$, $j$ odd\dotfill 37
  \item $\monjpr$, for $\mon$ in $\posv$, $j$ odd\dotfill 33
  \item $\mon_k$, for monomial $\mon$ in $\andposv$\dotfill 45
  \item $\mon_k$, for monomial $\mon$ in $\posv$\dotfill 33
  \item $\mon_k\ext$, for monomial $\mon$ in $\posv$\dotfill 38
  \item $\mon_{k,k+1}$, for monomial $\mon$ in $\andposv$\dotfill 48
  \item $\monkpr$, for monomial $\mon$ in $\posv$\dotfill 33
  \item $\smv$\dotfill 17
    \subitem modifications\dotfill \see{Notation~\ref{n.explain}}{17}
  \item $\smvadv$\dotfill 17
  \item $\smvw$\dotfill 14
  \item ${\rm SO}(V)$\dotfill 6
  \item $\mon'$, for monomial $\mon$ in $\posv$\dotfill 34
  \item standard monomial\dotfill 13
    \subitem $v$-compatible\dotfill 14
    \subitem $w$-dominated\dotfill 13
  \item $\mon\up$, for a monomial $\mon$\dotfill 24
  \item $\monsupjjpone$, for monomial $\mon$ in $\posv$\dotfill 31
  \item $\mon^k$, for monomial $\mon$ in $\andposv$\dotfill 45
  \item $S^w(v)(m)$\dotfill 10
  \item $\monw$, $w$ in $\idd$ or $I(d,n)$\dotfill 20, 47
  \item $\monwsubjjpone$, $w$ in~$\id$, $j$ odd\dotfill 41
  \item $\mon_w^j$, $w$ in~$\id$, $j$ odd\dotfill 41
  \item symmetric (monomial of $\andposv$)\dotfill 21

  \indexspace

  \item $T$, a specific maximal torus\dotfill 7
  \item $\tv$, set of monomials in $\posv$\dotfill 17
    \subitem modifications\dotfill \see{Notation~\ref{n.explain}}{17}
  \item tail, of a $v$-chain\dotfill 10
  \item $\mont$, fixed monomial in~$\posv$ in~\S\ref{s.ophi}%\dotfill 
		\ignore{41}
  \item truly orthogonal at $j$ ($j$ odd)\dotfill 33
  \item $\montwjjpone$\dotfill 41
  \item $\montwjjponehashstar$\dotfill 42
  \item $\montwjjponestar$\dotfill 43
  \item $\montwstar(:=\ophi(w,\mont))$\dotfill 43
  \item type (V, H, S), of an element in a $v$-chain\dotfill 22--23

  \indexspace

  \item $\uv$, set of monomials in $\rootsv\setminus\posv$\dotfill 17
    \subitem modifications\dotfill \see{Notation~\ref{n.explain}}{17}
  \item $u^*$, for $u\in\id$\dotfill 18

  \indexspace

  \item $V$, vector space of dimension $n$\dotfill 6
  \item $v$, fixed element of $I(d)$\dotfill 9
  \item $v$-chain\dotfill 10
  \item $v$-degree\dotfill 15
  \item vertical projection $p_v(\alpha)$\dotfill 21

  \indexspace

  \item $w(C)$ (or $w_C$), where $C$ is $v$-chain\dotfill 10
  \item $w^\hash$, for $w$ an element of $\idd$\dotfill 20
  \item $w(k)$\dotfill 33
  \item $(w,\mon')(:=\opi(\mon))$, for $\mon$ in $\posv$\dotfill 33, 34
  \item $w^*$, for $w$ an element of $\idd$\dotfill 20
  \item $\wsubjjpone$, $j$ odd\dotfill 41
  \item $\wsupj$, $j$ odd\dotfill 41

  \indexspace

  \item $X(w)$, Schubert variety\dotfill 9
  \item $x_k$, $x^k$, $x_{k,k+1}$, for $x\in I(d,n)$\dotfill 47--48
  \item $X_{r,c}$, variable\dotfill 15

  \indexspace

  \item $Y(w)(:=X(w)\cap\affinev)$\dotfill 14

\end{theindex}


==> scratch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% For purposes of switching indexing on and off:
%%%%%%%%%%%%%%  Choose the correct option of the \indexignore command
%%%%%%%%%%%%    defined below
%\newcommand{\indexignore}[1]{}
\newcommand{\indexignore}[1]{#1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  INDEXING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\indexignore{%%%%%%%%%%%%%%% For purposes of switching indexing on and off:
%%%%%%%%%%%%%%%%%%%%  Choose the correct option of the \indexignore command
	%%%%%%%%%%%%%%%%%%    defined above
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% For Indexing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{mymakeidx,showidx,robustindex}
\usepackage{mymakeidx,showidx}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% mymakeidx is a changed form of the standard makeidx.
%%%  The lines defining \see and \printindex have been
%%% changed from newcommands to providecommands.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%showidx (to show indexed entries in the margins)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{titletoc} % does not seem to work with amsbook option
%\usepackage[nottoc]{tocbibind} % does not seem to work with amsbook option
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% For indexing in color %%%%%%%%%%%%%%%%%
%\usepackage{color}
%\newcommand{\texdir}{/afs/ictp/home/k/kraghava/Latex}
%%%%%%%  Comments about some of the commands defined below:
% "defind" stands for font/color style of page numbers on which
% a concept is defined.  
% "impind" stands for font/color style of page numbers on which
% something important regarding the concept appears.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand\indexdub[1]{\index{#1}}  %can be changed later
%%% "indexdub" stands for "index-dubious".    Use this command
%%% to "index" something you are not sure you want to index,
%%%  then can later change it if you change your mind.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{\texdir/Definitions/rgb.tex}
\input{rgb.tex}
\newcommand\defind[1]{{\color{DarkGreen}{\ttfamily\itshape #1}}}
%\newcommand\defindmild[1]{{\color{DarkOrange}{\ttfamily\itshape #1}}}
\newcommand\defindmild{\defind}
\newcommand\impindmild[1]{{\color{DarkKhaki}\textit{#1}}}
%\newcommand\defind[1]{\textbf{#1}}
\newcommand\impind[1]{{\color{DarkBlue}{\itshape\bfseries #1}}}
%\newcommand\impind[1]{\textit{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\indexdub[1]{\index{#1}}  %can be changed later
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%The following copied from page 682 of the Companion 2nd edn
	%for making multiple indexes.  Later modified to suit our needs.
	%Comments are a summary of material found on page 681 Ibid.
%\show\markboth   
%%%  The pair of \show\markboth was used because index package
%%% warns that \markboth has changed.
		%\RequirePackage{index}
		\usepackage{index}
%\show\markboth
		% A starred form of the index command, that is,
		%\index*{foo} is introduced by the package (among
		% other things).
		%Its argument, in addition to being entered into the index,
		%is also typeset.
	%WARNING:  With standard LaTeX,  \index{\command} will sometimes
	%the expansion of the command into the .idx file.   With the index
	%package, \index{\command} itself is written.    This might lead
	%to unexpected results.   Be careful and check to see if what you
		%get is what you meant.
		%\proofmodetrue		%while proofing the index entries
					%like showidx package
		\indexproofstyle{\footnotesize\tiny}	
				%customizing the size and shape of
				%the font used in the margins
		\shortindexingon %This allows you to write ^{foo} for
				%\index{foo} and _{foo} for \index*{foo}.
		%  (in the index package)
					%Shorthand not available in math mode
				%for underscore and circumflex have special
					%meanings there.
	% knr's comment:   shortindexing didn't work very well.  
		%  it is not used in the document.

		\newindex{n}{ndx}{nnd}{Index of Notation}
			%This defines a new index, namely the one for
			%notations.   Explanation:
			% n is the "tag" (name of the index)
			% ndx is the raw-ext (the extension of the file
			%into which latex will write the index
			%entries.
			% nnd is extension of the final latex file containing
			%the index and which latex will read and print
			%at the point that it encounters the
			%\printindex[n] command.
			% Index of Notations:  what will be printed on
			% top of the Index page.
	%Here are the examples from the Companion which were used to produce
			%the Companion itself.
		%\newindex{xauthor}{adx}{and}{People}
		%\newindex{xcmds}{cdx}{cnd}{Index of Commands and Concepts}
	%What happens to the \makeindex command that you use in the preamble
		%in standard latex?     Well,   the index is produced by
		%running makeindex -o file.nnd -t file.nlg file.ndx 
		%The -t option is to name of the "log" file (into which the
		%transcript of the makeindex run is written).
		%This is much like running bibtex.
		\makeindex 	%This is necessary to make the index
				%in standard latex (without the index package).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{afterpage,repeatindex} % for repeatindex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% afterpage is only there because it is required by repeatindex.
% The idea of repeatindex is a nice one:   if there is a pagebreak or
% a column break between the main entry of an index and a subitem,  it
%  will write the main entry on the next page/column.    It either didn't
% work at all, or, if it did,  it produced three dots ... at the head of
% every column,  regardless of whether there was a break or not.
% Possible reason for why repeatindex did not work:  it needs its own
% .ist.    Trying to merge the few lines in repeatindex.ist with my
% own .ist was the problem.   There seems to be some conflict between
% the index package and repeatindex.
%%%%%%%%    Gave up on repeatindex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Indexing Commands Over %%%%%%%%%%%%%%%
}    %   End of \indexignore
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setstretch{1.0}
%\renewcommand\see[2]{\\ \textit{see\/} #1}
%\renewcommand\see[2]{\\ {\small \textsc{see\/} #1}}
\renewcommand\see[2]{{\small \textsc{see\/} #1}}
\newcommand\seeindn[2]{{\small \textsc{see\/} #1}}
\newcommand\sameas[2]{{\small \textsc{same as\/}} #1}
%\renewcommand\seealso[2]{{\small \textsc{see\/} #1}}
\newcommand\seealsoindn[2]{\textit{see also\/} #1 in index of notation}
%\newcommand\seemainind[2]{\defind{#2}, \textit{see also\/} main index}%
			%#1 in main index}
\newcommand\seemainind[2]{\defind{#2}, see also \textit{#1\/}%
		in the main index}
\newcommand\seemainindsame[1]{\defind{#1}}%, see also the main index}
%\renewcommand\seealso[2]{\\ {\small \textsc{see also\/} #1}}
\renewcommand\seealso[2]{{\small \textsc{see also\/} #1}}
%\renewcommand\seealso[2]{{\footnotesize \textsc{see also\/} #1}}
%\renewcommand\see[2]{\\ \textit{see also\/} #1}
\newcommand\impindseealso[2]{\impind{#2}, \textit{see also\/} #1}
\newcommand\indnotation[2]{#1}
\providecommand\gitmod{{/\negthinspace\negthinspace/}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   The following is important:   The Companion is incomplete about this.
%   The \printindex takes two optional arguments.   The first is to
%   decide which index to print and the second for text that goes write
%   after the heading but before any entries.    We wanted a few lines
%   of explanation after the heading but before the entries.   This
%   was not easy to do.   In some situations,  putting the desired text
%   into the \IndexPrologue as follows worked:
%\IndexPrologue{Does this go on top of the Index?  Bingo!}
%    But once again,  this didn't work with the index package.
%    So the above solution was found out.   It was not easy to find it.
%    We obtained it by looking at various definitions (by means of \show).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% Index (the main one) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\printindex[default][%
\addtocontents{mtc}%
	{\protect\contentsline{chapter}{\protect\tocchapter{}%
	{}{Index\hspace{3pt}\protect\dotfill\ }}{\thepage}}
Page numbers appear in three fonts,  two special fonts in addition 
to the ordinary one.   For example,  consider the index
entry ``extremal weight vectors''.    The appearance of the page number
\defind{23\/} means that the definition of extremal weight vectors
can be found on that page.     As another example,  consider the
index entry ``first basis theorem''.    The appearance of 
the page number \impind{189\/} means that the statement of the theorem
can be found on that page.\vskip-2cm]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Index of notation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\printindex[n][%
\addtocontents{mtc}%
	{\protect\contentsline{chapter}{\protect\tocchapter{}%
	{}{Index of Notation\hspace{3pt}\protect\dotfill\ }}{\thepage}}]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

